Bi-Lipschitz invariance of the multiplicity

The multiplicity of an algebraic curve $C$ in the complex plane at a point $p$ on that curve is defined as the number of points that occur at the intersection of $C$ with a general complex line that passes close to the point $p$. It is shown that $p$ is a singular point of the curve $C$ if and only if this multiplicity is greater than or equal to 2, in this sense, such an integer number can be considered as a measure of how singular can be a point of the curve $C$. In these notes, we address the classical concept of multiplicity of singular points of complex algebraic sets (not necessarily complex curves) and we approach the nature of the multiplicity of singular points as a geometric invariant from the perspective of the Multiplicity Conjecture (Zariski 1971). More precisely, we bring a discussion on the recent results obtained jointly with Lev Birbrair, Javier Fern\'andez de Bobadilla, L\^e Dung Trang and Mikhail Verbitsky on the bi-Lipschitz invariance of the multiplicity.

==> bibliography.tex <==

\begin{thebibliography}{99}

% \bibitem{Barden}
% Barden, D. 
% {\it Simply connected five-manifolds}. 
% Ann. of Math., vol. 82 (1965), no. 2, 365--385.

% \bibitem{BernigL:2007} 
% {Bernig, A. and Lytchak, A.}  
% {\it Tangent spaces and Gromov-Hausdorff limits of subanalytic spaces}. 
% J. Reine Angew. Math., vol. 608 (2007), 1--15.

\bibitem{BirbrairFLS:2016}
{Birbrair, L.; Fernandes, A.; L\^e D. T. and Sampaio, J. E.}
{\it Lipschitz regular complex algebraic sets are smooth}.
Proceedings of the American Mathematical Society, vol. 144 (2016), no. 3, 983--987.

% \bibitem{BirbrairF:2000}  
% {Birbrair, L.; Fernandes, A.} 
% {\em Metric theory of semialgebraic curves}, 
% Rev. Mat. Complut., vol. 13 (2000), no. 2, 369--382.

% \bibitem{BirbrairFG:2017}
% {Birbrair, L.; Fernandes, A. and Grandjean, V.}
% {\it Thin-thick decomposition for real definable isolated singularities}.
% Indiana University Math. J., vol. 66 (2017), 547--557.

% \bibitem{BirbrairFN} 
% {Birbrair, L.; Fernandes, A. and Neumann, W. D.} 
% {\it Normal embedding of complex algebraic surfaces}. 
% Real and Complex Singularities. LMS Lecture Note Series 380 (2010), 17--21.

\bibitem{BirbrairFSV:2020}
{Birbrair, L.; Fernandes, A.; Sampaio E. and  Verbitsky, M.}
{\it Multiplicity of singularities is not a bi-Lipschitz invariant.}
Mathematische Annalen 377 (2020), 115--121 

% 
% \bibitem{BirbrairG}
% {Birbrair, L. and Gabrielov, A.}
% {\it Ambient Lipschitz equivalence of real surface singularities}.
% International Mathematics Research Notices, vol. 2019 (2019), no. 20,  6347–-6361.


% 
% \bibitem{BirbrairM:2018}
% {Birbrair, L. and Mendes, R.} 
% {\em Arc criterion of normal embedding}.
% Singularities and foliations. geometry, topology and applications, 549–553, Springer Proc. Math. Stat., 222, Springer, Cham, 2018. 

% \bibitem{BirbrairM:2000} 
% {Birbrair, L. and Mostowski, T.}
% {\em Normal embeddings of semialgebraic sets}.
% Michigan Math. J., vol. 47 (2000), 125-132.

% \bibitem{Bishop:1964}
% {Bishop, E.} 
% {\it Condition for the analyticity of certain sets}. 
% Michigan Math. J., vol. 11 (1964), 289-304. 

\bibitem{BobadillaFS}
{Bobadilla, J. F., Fernandes, A. and Sampaio, J. E.}
{\it Multiplicity and degree as bi-Lipschitz invariants for complex sets}.
Journal of Topology, vol. 11 (2018), no. 4, 958--966.

% \bibitem{Brieskorn:1966} 
% {Brieskorn, E. V.} 
% {\it Examples of singular normal complex spaces which are topological manifolds}.
% Proc. Nat. Acad. Sci. U.S.A., vol. 55 (1966), 1395--1397.

\bibitem{BierstoneM:1988} 
Bierstone, E. and Milman, P.D.
{\it Semianalytic and subanalytic sets}.
Publications math\'ematiques de l'I.H.\'E.S., vol. 67 (1988), 5--42.

\bibitem{Chirka:1989} 
{Chirka, E. M.} 
{\it Complex analytic sets}.
Kluwer Academic Publishers, 1989.

\bibitem{Comte:1998}
{Comte, G.}
{\em Multiplicity of complex analytic sets and bi-Lipschitz maps}.
Real analytic and algebraic singularities (Nagoya/Sapporo/Hachioji, 1996) Pitman Res. Notes Math. Ser. 381 (1998),  182--188.

\bibitem{ComteMT:2002}
{Comte, G.; Milman, P. and Trotman, D.}
{\em On Zariski's multiplicity problem}.
Proceedings of the American Mathematical Society 130 (2002), no. 7, 2045--2048.

% \bibitem{Coste:1966} 
% {Coste, M.} 
% {\it An introduction to O-minimal Geometry}.
% Institut de Recherche Math\'ematique de Rennes, 1999.

% \bibitem{Crowley:manifolds}
% {Crowley, D.}. 
% {\it 5-manifolds: 1-connected}.
% Bulletin of the Manifold Atlas (2011), 49--55. 

\bibitem{Dimca:1992}
{Dimca, A.}
{\it Singularities and topology of hypersurfaces}.
New york: Springer-Verlag, 1992.

\bibitem{Draper:1969} 
{Draper, R. N.}
{\it Intersection Theory in Analytic Geometry}.
Mathematische Annalen, vol. 180 (1969), 175--204.

% \bibitem{Dries:1998}
% {van den Dries, L.}
% {\em Tame topology and o-minimal structures.}
%  London Mathematical Society Lecture Note Series, 248, Cambridge University Press, Cambridge, 1998.

\bibitem{Ephraim:1976a} 
{Ephraim, R.}
\newblock {\it $C^1$ preservation of multiplicity}. 
\newblock Duke Math., vol. 43 (1976), 797--803.


% \bibitem{Ephraim:1976b}
% {Ephraim, R.}
% {\it The cartesian product structure and {C}$^\infty$ equivalences of singularities}.
% Trans. Amer. Math. Soc., vol. 224 (1976), no. 2, 299--311.

% \bibitem{Eyral:2007} 
% {Eyral, C.}
% {\em Zariski's multiplicity questions - A survey}.
% New Zealand Journal of Mathematics, vol. 36 (2007), 253--276.

\bibitem{F}
{Fernandes, A.}
{\it Topological equivalence of complex curves and bi-Lipschitz maps}.
{Michigan Math. J., vol. 51 (2003), 593--606}.

\bibitem{FernandesS:2016}
{Fernandes, A. and Sampaio, J. E.}
{\it Multiplicity of analytic hypersurface singularities under bi-Lipschitz homeomorphisms}.
Journal of Topology, vol. 9 (2016), 927--933.

\bibitem{FSS}
{Fernandes, A.; Sampaio, J. E. and Silva, J. P.} 
{\it H\"older equivalence of complex analytic curve singularities.} 
Bull. London Math. Soc., vol. 50 (2018), no. 5, 874-886.


% \bibitem{FernandesS:2019}
% {Fernandes, A. and Sampaio, J. E.}
% {\it Tangent cones of Lipschitz normally embedded sets are Lipschitz normally embedded. Appendix by Anne Pichon and Walter D. Neumann}.
% International Mathematics Research Notices, vol. 2019 (2019), no. 15, 4880-4897.

% \bibitem{FernandesS:2020}  
% {Fernandes, A. and Sampaio, J. E.}
% {\em On Lipschitz rigidity of complex analytic sets}. 
% The Journal of Geometric Analysis, vol. 30 (2020), 706--718.
% 
% \bibitem{FernandesS:2021}  
% {Fernandes, A. and Sampaio, J. E.} 
% {\em On characterization of smoothness of complex analytic sets}.
% Preprint (2021), \url{https://www.researchgate.net/publication/337060534_ON_CHARACTERIZATION_OF_SMOOTHNESS_OF_COMPLEX_ANALYTIC_SETS}

% \bibitem{Bobadilla:2005} 
% {Fern\'andez-Bobadilla, J.} 
% Answers to some equisingularity questions, 
% Invent. math., vol. 161 (2005), 657--675.

\bibitem{Gau-Lipman:1983}
{Gau, Y.-N. and Lipman, J.}
{\it Differential invariance of multiplicity on analytic varieties}.
Inventiones mathematicae, vol. 73 (1983), no. 2, 165--188.

\bibitem{JongP:2000}
de Jong, T. and Pfister, G.
{\it Local Analytic Geometry Basic Theory and Applications}.
Springer Fachmedien Wiesbaden , 2000

% \bibitem{KapovichK:2014}
% Kapovich, M. and Koll\'ar, J.
% {\it Fundamental groups of links of isolated singularities.}
% Journal of the American Mathematical Society, vol. 27 (2014), n. 4, 929--952.

% \bibitem{KatoM:1975}
% Kato, M. and Matsumoto, Y.
% {\it On the connectivity of the Milnor fiber of a holomorphic function at a critical point.}
% Manifolds, Tokyo 1973 (Proc. Internat. Conf., Tokyo, 1973), pp. 131--136. Univ. Tokyo Press, Tokyo, 1975.

% \bibitem{KernerPR:2018}
% {Kerner, D.; Pedersen, H. M. and Ruas, M. A. S.}
% {\em Lipschitz normal embeddings in the space of matrices}. 
% Math. Z., vol. 290 (2018), no. 1-2, 485--507.

\bibitem{Kirszbraun:1934} 
{Kirszbraun, M.} 
{\it $\ddot{U}$ber die zusammenziehende und Lipschitzsche Transformationen}. 
Fundamenta Math., vol. 22 (1934), no. 1, 77--108.

% \bibitem{Koike:2010} 
% {Koike, S.; Loi , Ta Le; Paunescu, L. and Shiota, M.}
% {\it Directional properties of sets definable in o-minimal structures}.
% Ann. Inst. Fourier (Grenoble), vol. 63 (2013), no. 5, 2017--2047.

% \bibitem{Koike:2009} 
% {Koike, S. and Paunescu, L.} 
% {\it The directional dimension of subanalytic sets is invariant under bi-Lipschitz homeomorphisms}.
% Ann. Inst. Fourier (Grenoble), vol. 59 (2009), no. 6, 2445--2467.

% \bibitem{Koike:2013} 
% {Koike, S. and Paunescu, L.} 
% {\it On the Geometry of sets satisfying the se\-quen\-ce se\-lec\-tion property}.
% J. Math. Soc. Japan, vol. 67 (2015), no. 2, 721--751.
% 
% \bibitem{Kollar:Seifert_}
% {Koll\'ar, J.} 
% {\it Seifert Gm-bundles}. 
% arXiv:math/0404386v2 [math.AG], (2004).
% 
% \bibitem{Kollar:circle_}
% {Koll\'ar, J.}
% {\it Circle actions on simply connected 5-manifolds,}
% Topology, vol. 45 (2006), no. 3, 643--671. 
 
% \bibitem{Kurdyka:1992}
% {Kurdyka, K.}
% {\em On a subanalytic stratification satisfying a Whitney property with exponent 1}.
% Lecture Notes in Math., 1524, 316--323. Berlin: Springer-Verlag, 1992.

\bibitem{Kurdyka:1997} 
{Kurdyka, K. and Orro, P.}
{\em Distance g{\'e}od{\'e}sique sur un sous-analytique}.
Rev. Mat. Complut., vol. 10 (1997), no. Suplementario, 173--182.

% \bibitem{Kurdyka:1989} 
% {Kurdyka, K. and Raby, G.}
% {\it Densit\'e des ensembles sous-analytiques}. 
% Ann. Inst. Fourier (Grenoble), vol. 39 (1989), no. 3, 753--771.

\bibitem{Le:1973} 
{L\^e D. T.}
{\it Topologie des singularit\'es des hypersurfaces complexes}. 
(French) Singularit\'es \`a  Carg\`ese, Asterisque, vol. 7 and 8 (1973), 171--182.

% \bibitem{Le:1973b} 
% {L\^e D. T.}
% {\it Calcul du nombre de cycles \'evanouissants d'une hypersurface complexe}. 
% (French) Ann. Inst. Fourier (Grenoble), vol. 23 (1973), no. 4, 261--270.

% \bibitem{Le:1980} 
% {L\^e D. T.}
% {\it Ensembles analytiques complexes avec lieu singulier de dimension un}. 
% (D'Apres I. N. Iomdine), Seminar on Singularities (Paris, 1976/1977), Publ. Math. Univ. Paris VII, vol. 7 (1980),
% 87--95.

% \bibitem{Massey:1995}
% {Massey, D. B.}
% {\it L\^e cycles and hypersurfaces singularities}.
% Lecture Notes Math., vol. 1615, Berlin: Springer-Verlag, 1995.

\bibitem{Massey:2017}
{Massey, D. B.}
{\it A New Conjecture, a New Invariant, and a New Non-splitting Result}. 
J.L. Cisneros-Molina et al. (eds.), Singularities in Geometry, Topology, Foliations and Dynamics,
Trends in Mathematics, Springer International Publishing, 171-181.

\bibitem{Mcshane:1934} 
{Mcshane, E. J.} 
{\it Extension of range of functions}.
Bull. Amer. Math. Soc., vol. 40 (1934), 837--842.

\bibitem{Milnor:1968}
{Milnor, J.}
{\it Singular points of complex hypersurfaces}.
Princeton: Princeton University Press, 1968.

% \bibitem{Milnor:1974} %
% {Milnor, J. W. and Stasheff, J. D.} 
% {\it Characteristics Classes}.
% In Annals of mathematics studies, vol. 76. Princeton University Press, 1974.

\bibitem{Mo}
{ Mostowski, T.}
{\it Lipschitz equisingularity}, 
Dissertationes Math. (Rozprawy Mat.) 243 (1985).


% \bibitem{M} 
% {Mumford, D.} 
% {\it The topology of normal singularities of an algebraic surface and a criterion for simplicity}.
% Inst. Hautes \'Etudes Sci. Publ. Math., vol. 9 (1961), 5--22.
  
% \bibitem{Munkres:2014}
% {Munkres, J.}
% {\it Topology,}
% 2nd ed. Harlow: Pearson Education Limited, 2014.

\bibitem{NeumannP:2012}
{Neumann, W. and Pichon, A.}
{\it Lipschitz geometry of complex surfaces: analytic invariants and equisingularity.}
arXiv:1211.4897v3 [math.AG] (2012), pp 61.

\bibitem{N-P}
{Neumann, W. and Pichon, A.}
{\it Lipschitz geometry of complex curves}.
Journal of Singularities, vol. 10 (2014), 225--234.

% \bibitem{Parusinski:1988}
% {Parusinski, A.}
% {\em Lipschitz properties of semianalytic sets}.
% Ann. Inst. Fourier, vol. 38 (1988), 189--213.

\bibitem{Parusinski:1994}
{Parusinski, A.}
{\it Lipschitz stratification of subanalytic sets}.
Ann. Sci. \'Ecole Norm. Sup. (4) 27 (1994), 661--696.

% \bibitem{Pawlucki:1985}
% {Paw\l ucki, Wies\l aw.}
% {\it Quasi-regular boundary and Stokes' formula for a sub-analytic leaf}.
% In: \L awrynowicz J. (eds) Seminar on Deformations. Lecture Notes in Math., vol 1165. Berlin, Heidelberg: Springer. 1985.

\bibitem{P-T}
{Pham, F. and Teissier, B.}
{\it Fractions lipschitziennes d'une alg\`ebre analytique complexe et saturation de Zariski}.
Centre de Math\'ematiques de l'Ecole Polytechnique (Paris), June 1969.

\bibitem{Prill:1967} 
{Prill, D.}
{\it Cones in complex affine space are topologically singular}.
Proc. of Amer. Math. Soc., vol. 18 (1967), 178-182.

\bibitem{Randell:1979}
{Randell, R.}
{\it On the topology of non-isolated singularities}.
Geometric Topology. Academic Press, New York-London (1979), 445--473.

\bibitem{RislerT:1997}
{Risler, J.-J. and Trotman, D.}
{\em Bi-Lipschitz invariance of the multiplicity}.
Bull. London Math. Soc. 29 (1997), 200--204.

\bibitem{Sampaio:2016}
{Sampaio, J. E.}
{\it Bi-Lipschitz homeomorphic subanalytic sets have bi-Lipschitz homeomorphic tangent cones}.
Selecta Math. (N.S.), vol. 22 (2016), no. 2, 553-559.

\bibitem{Sampaio:2019}
{Sampaio, J. E.}
{\it On Zariski's multiplicity problem at infinity}.
Proc. Amer. Math. Soc., vol. 147 (2019), 1367-1376.

\bibitem{Sampaio:2020}
{Sampaio, J. E.}
{\it Multiplicity, regularity and blow-spherical equivalence of complex analytic sets.}
The Asian Journal of Mathematics, vol. 24 (2020), no. 5, 803-820.

% \bibitem{Smale}
% {Smale, S.} 
% {\it On the structure of 5-manifolds,}
% Ann. of Math., vol. 75 (1962), no. 2, 38-46.

% \bibitem{Stoll:1964a}
% {Stoll, W.}
% {\it The growth of the area of a transcendental analytic set. I}.
% Math. Ann., 156 (1964), no. 1, 47-78.

% \bibitem{Stoll:1964b}
% {Stoll, W.}
% {\it The growth of the area of a transcendental analytic set. II}.
% Math. Ann., vol. 156 (1964), 144-170. 

\bibitem{Trotman:1977} 
{Trotman, D.}
\newblock {\it Multiplicity is a $C^1$ invariant}. 
\newblock University Paris 11 (Orsay), Preprint (1977).

% \bibitem{Trotman:1998} 
% {Trotman, D.}
% \newblock {\it Multiplicity as a $C^1$ invariant}.
% In: Real analytic and algebraic singularities (Nagoya/Sapporo/Hachioji, 1996). Pitman Research Notes in Mathematics Series, vol. 381, pp. 215--
% 221. Longman, Harlow. 1998.

% \bibitem{Valette:2007} 
% {Valette, G.}
% {\em The link of the germ of a semi-algebraic metric space}. 
% Proc. Amer. Math. Soc., vol. 135 (2007), no. 10, 3083-3090.

% \bibitem{Valette:2010} 
% {\it Valette, Guillaume}. 
% {\it Multiplicity mod 2 as a metric invariant}. 
% Discrete Comput. Geom., vol. 43 (2010), 663--679.

% \bibitem{Weibel:1994}
% {WEIBEL, C. A.}
% {\em An introduction to homological algebra}. 
% Cambridge University Press, 1994.

\bibitem{Whitney:1934}
{Whitney, H.}
{\it Analytic extensions of functions defined in closed sets}.
Transactions of the Amer. Math. Soc., vol. 36 (1934), 63--89.

\bibitem{Whitney:1965a} 
{Whitney, H.}
{\it Tangents to an analytic variety}. 
Annals of Mathematics 81 (1965), no. 3, 496--549.

\bibitem{Whitney:1965b} 
{Whitney, H.}
{\it Local properties of analytic varieties}.
Differential and Combinatorial Topology, Princeton Univ. Press, (1965), 205--244.

\bibitem{Whitney:1972} 
{Whitney, H.}
{\it Complex Analytic Varieties}.
Addison-Wesley publishing company, Mass.-Menlo Park, Calif.-London-Don Mills, Ont, 1972.

% \bibitem{Whyburn:1935}
% {Whyburn, G. T.}
% {\it On sequence and limiting sets.}
% Fundamenta Mathematicae, vol. 25 (1935), 408--426.

\bibitem{Zariski:1971} 
{Zariski, O.}
{\it Some open questions in the theory of singularities}. 
Bull. of the Amer. Math. Soc. 77 (1971), no. 4, 481--491.
\end{thebibliography}

